SelfPose3d: Self-Supervised Multi-Person Multi-View 3d Pose Estimation

We present a new self-supervised approach, SelfPose3d, for estimating 3d poses of multiple persons from multiple camera views. Unlike current state-of-the-art fully-supervised methods, our approach does not require any 2d or 3d ground-truth poses and uses only the multi-view input images from a calibrated camera setup and 2d pseudo poses generated from an off-the-shelf 2d human pose estimator. We propose two self-supervised learning objectives: self-supervised person localization in 3d space and self-supervised 3d pose estimation. We achieve self-supervised 3d person localization by training the model on synthetically generated 3d points, serving as 3d person root positions, and on the projected root-heatmaps in all the views. We then model the 3d poses of all the localized persons with a bottleneck representation, map them onto all views obtaining 2d joints, and render them using 2d Gaussian heatmaps in an end-to-end differentiable manner. Afterwards, we use the corresponding 2d joints and heatmaps from the pseudo 2d poses for learning. To alleviate the intrinsic inaccuracy of the pseudo labels, we propose an adaptive supervision attention mechanism to guide the self-supervision. Our experiments and analysis on three public benchmark datasets, including Panoptic, Shelf, and Campus, show the effectiveness of our approach, which is comparable to fully-supervised methods. Code: https://github.com/CAMMA-public/SelfPose3D. Video demo: https://youtu.be/GAqhmUIr2E8.

==> macros.tex <==
\usepackage{xcolor}
\usepackage{wrapfig}
\usepackage{soul}

\definecolor{yellow}{rgb}{1,1, 0.6}
\definecolor{lightyellow}{rgb}{1,1, 0.8}
\definecolor{orange}{rgb}{1, 0.8, 0.6}
\definecolor{coral}{RGB}{246,131,65}
\definecolor{pinkred}{rgb}{1, 0.6, 0.6}
\definecolor{hotpink}{RGB}{238,64,195}
\definecolor{lavender}{RGB}{207,226,243}
\definecolor{gainsboro}{RGB}{208,224,227}
\definecolor{gainsboro2}{RGB}{217,234,211}
\definecolor{blanchedalmond}{RGB}{252,229,205}

\newcommand{\missfigure}{\textcolor{red}{[F]}}
\newcommand{\misscite}{\textcolor{red}{[C]}}
\newcommand{\missref}{\textcolor{red}{[R]}}

\newcommand{\ray}[1]{{\textcolor{red}{#1}}}
\newcommand{\todo}[1]{{\textcolor{red}{(TODO: #1)}}}

\newcommand{\model}{XXXX}
\newcommand{\modelname}{XXXX\xspace}

\newcommand{\coverage}{spatial coverage\xspace}
\newcommand{\complexity}{detail complexity\xspace}
%altitude or distance
\newcommand{\altitude}{distance\xspace}
\newcommand{\altitudefull}{distance to the scene\xspace}
\newcommand{\altitudes}{distances\xspace}
\newcommand{\altitudesfull}{distances to the scene\xspace}

\newcommand{\copyrightgoogle}{\href{https://www.google.com/help/terms_maps/}{\textcopyright 2022 Google}\xspace}

==> sec/1_intro_bkp.tex <==
\section{Introduction}
\label{sec:intro}

\begin{figure*}[t!]
	\centering
	\begin{subfigure}[t]{0.43\textwidth}
		\centering
		\includegraphics[width=0.95\linewidth]{figures/figure_intro_a.jpg}
	\end{subfigure}
	\begin{subfigure}[t]{0.56\textwidth}
		\centering
		\includegraphics[width=0.94\linewidth]{figures/figure_intro_b.jpg}
	\end{subfigure}
	\caption{\small{Our self-supervised approach, called SelfPose3d, estimates multi-person 3d poses from multi-view images and pseudo 2d poses generated using an \emph{off-the-shelf} 2d human pose estimator. We propose a self-supervised learning objective that generates differentiable and geometrically constrained 2d joints and heatmaps across multiple views from bottleneck 3d poses. On the right, we show 3d pose outputs from our approach along with estimated body meshes (using SMPL body mesh fitting on 3d poses \cite{loper2015smpl,bogo2016keep}) and the projected 2d poses.}}
	\label{fig:intro-fig}
	\vspace{-3mm}
\end{figure*}


The growing interest in computer vision to alleviate the dependence on ground truth labels has enabled the emergence of self-supervised learning approaches that use no ground-truth supervision for various downstream tasks \cite{jakab2018unsupervised,jakab2020self,caron2021emerging,bhatnagar2020loopreg}. This paper proposes a self-supervised method, \emph{SelfPose3d}, for estimating the 3d poses of multiple people interacting in a complex scene captured from a few calibrated cameras. In particular, using only multi-view images and pseudo 2d poses generated from an \emph{off-the-shelf} human pose detector as input, we aim to automatically learn a deep neural network that can predict the 3d poses of all the persons. The task is challenging and so far the related work has only focused on developing fully-supervised approaches that use 3d ground-truth poses, generated from tens or hundreds of multi-view cameras \cite{joo2015panoptic,tu2020voxelpose,lin2021multi,zhang2021direct,wu2021graph,reddy2021tessetrack}. 

One key challenge in multi-view multi-person 3d pose estimation is establishing person correspondences across multiple views. Using these correspondences, the standard framework of multi-view geometry can be applied for reconstructing 3d poses from multi-view 2d poses utilizing triangulation and temporal refinement \cite{joo2014map,joo2015panoptic,pirinen2019domes}. However, these non-learning-based approaches require sufficiently dense camera systems for accurately solving person correspondences and reconstructing 3d poses \cite{joo2015panoptic}, leading to sizeable 3d pose reconstruction errors otherwise \cite{pirinen2019domes}. With dense camera systems, they provide accurate 3d pose reconstructions that have been used as ground-truth to train learning-based fully-supervised deep learning approaches relying only on a few cameras \cite{tu2020voxelpose,lin2021multi,zhang2021direct,wu2021graph,reddy2021tessetrack}. Such carefully constructed setups relying on large camera systems are however not always practical, especially in new unseen domains. In this work, we show that \emph{accurate 3d pose reconstruction of multiple persons can be achieved using only a few sparse multi-view cameras and without any 2d or 3d ground truth.}

We base our work on VoxelPose \cite{tu2020voxelpose} and modify the approach to make it fully self-supervised. VoxelPose constructs a voxel-based 3d feature space by un-projecting the 2d joints heatmap representations \cite{iskakov2019learnable}. It then uses the 3d feature space in a two-step approach, first to localize 3d roots (mid-hip joint) and establish the cross-view correspondence of the persons, and second, to perform 3d pose regression for each localized person. The first step uses 3d root ground-truth, and the second step uses full 3d pose ground-truth for learning. 

To circumvent the dependence on the ground-truth 2d and 3d poses, we firstly estimate pseudo 2d poses by running an \emph{off-the-shelf} human pose detector \cite{sun2019deep} on the training dataset. Then, we propose two self-supervised learning objectives: \textbf{\emph{self-supervised 3d root localization}} for person localization in 3d space and \textbf{\emph{self-supervised 3d pose estimation}} for the full 3d pose estimation of each localized person. Lastly, we apply an \textbf{\emph{adaptive supervision attention}} mechanism to alleviate the label inaccuracy. 

\paragraph{\textbf{Self-supervised 3d root localization}} VoxelPose uses a 3d feature space, from un-projected multi-view heatmaps of all the joints using \cite{iskakov2019learnable}. We hypothesize that using only 2d multi-view root-heatmaps is sufficient for 3d root localization. This allows us to establish a one-to-one relationship between 3d root joints and 2d multi-view root-heatmaps for self-supervising the root joint localization. Specifically, we randomly place 3d points in 3d world-space and project them to each view using the given camera parameters, subsequently rendering the projected 2d points as heatmap representations. This generates a synthetic dataset containing 3d points (roots) and their corresponding rendered multi-view root-heatmaps. We then use this dataset to train a 3d root localization model that takes multi-view root-heatmaps as input and predicts the 3d roots as output. We further regularize the model by enforcing invariant constraints between pairs of affine augmented root-heatmaps coming from the real multi-view input. 

\paragraph{\textbf{Self-supervised 3d pose estimation}} The above approach does not establish correspondences between the 3d roots and 2d root-heatmaps of the real-world multi-view input. Since there's no ground-truth 3d roots, we instead propose to use 3d poses as a bottleneck representation and recover the accurate underlying 3d poses using \emph{differentiable multi-view 2d representations} and \emph{cross-affine-view consistency}. In particular, given a multi-view input image, we apply two random affine augmentations and pass them to the 3d pose estimation model. It generates the bottleneck 3d poses corresponding to each affine augmented multi-view image. To enforce the model to learn and reason in the spatial dimension, we map the bottleneck 3d poses onto each view obtaining 2d joints, and render them into spatial heatmap representations in an end-to-end differentiable way. We further put tight geometric constraints by cross-affine-views operation, \emph{i.e.} the bottleneck 3d poses from the 1st affine augmented multi-view image is mapped and rendered in the 2nd affine augmented multi-view image space and vice versa. Finally, we use the affine transformed 2d joints and heatmaps from the 2d pseudo poses to enable the geometrically constrained learning, with both $L_1$ and $L_2$ losses. See \cref{fig:method} for a visual description of the overall approach.

\paragraph{\textbf{Adaptive supervision attention}} The pseudo 2d poses contain non-negligible noises (mostly due to occlusions), limiting the training result. To guide our model focus on more reliable regions or views, we apply two strategies towards $L_1$ and $L_2$ losses respectively. For $L_1$ loss supervision, we employ a hard attention, where we ignore the one view with the largest absolute error for each multi-view data. For $L_2$ loss supervision, we employ a soft attention. We use a lighter VoxelPose backbone to process each view, obtaining same-size attention heatmaps. During loss computation, we compute the element-wise product of the attention heatmaps and the square error before averaging. To avoid obtaining zero attention which the model tends to, we propose an adversarial training strategy, where we create tensors of all ones as the attention heatmap labels, and use $L_2$ loss as the attention loss. 

Evaluation on three 3d pose benchmarks datasets, Panoptic \cite{joo2015panoptic}, Shelf \cite{belagiannis20143d} and Campus \cite{belagiannis20143d}, along with extensive ablation studies on the Panoptic \cite{joo2015panoptic} dataset, show the effectiveness of our approach. Our approach reaches a performance comparable to fully-supervised approaches and performs significantly better than a non-learning based approach using triangulation. Finally, SMPL body mesh fitting \cite{loper2015smpl,bogo2016keep} on our estimated 3d poses generates geometrically plausible body shapes (see \cref{fig:intro-fig} and \cref{fig:qual_1}).

We summarize our contributions as follows: 1) We address the challenging multi-person multi-view 3d person pose estimation problem using a self-supervised approach without any 2d or 3d ground truth. 2) We propose \emph{self-supervised 3d root localization} to estimate the 3d root location utilizing synthetic 3d roots and the corresponding rendered multi-view root heatmaps. 3) We propose \emph{self-supervised 3d pose estimation} by using a new method to recover geometrically constrained 2d joints and heatmap representations from the bottleneck 3d poses. 4) We propose \emph{adaptive supervision attention} with an adversarial training strategy, to address the misinformation caused by the inaccurate pseudo labels.


